Grounding Visual Illusions in Language: Do Vision-Language Models Perceive Illusions Like Humans?

Vision-Language Models (VLMs) are trained on vast amounts of data captured by humans emulating our understanding of the world. However, known as visual illusions, human's perception of reality isn't always faithful to the physical world. This raises a key question: do VLMs have the similar kind of illusions as humans do, or do they faithfully learn to represent reality? To investigate this question, we build a dataset containing five types of visual illusions and formulate four tasks to examine visual illusions in state-of-the-art VLMs. Our findings have shown that although the overall alignment is low, larger models are closer to human perception and more susceptible to visual illusions. Our dataset and initial findings will promote a better understanding of visual illusions in humans and machines and provide a stepping stone for future computational models that can better align humans and machines in perceiving and communicating about the shared visual world. The code and data are available at https://github.com/vl-illusion/dataset.

==> A-2-related-work.tex <==
\section{Related Work}

\paragraph{Human Visual Illusion and Its Evaluation} 
Visual illusions in humans are instances where human subjective perceived properties, such as color, size, and lightness, 
deviates from their true physical characteristics~\citep{carbon2014understanding}.
 This underscores the fact that the human brain doesn't perfectly replicate physical features; rather, it integrates contextual information and prior knowledge to form the perceptual experiences \citep{carbon2014understanding}.
Visual illusions have been a prominent topic within cognitive psychology and neuroscience, with systematic deliberations dissecting various categories of these illusions \citep{robinson2013psychology, shapiro2016oxford}. Debates regarding the underlying processes of visual illusions center on two primary theories: one posits that top-down influences, such as an observer's prior knowledge and experiences, significantly impact visual processing \citep{teufel2018prior, caporuscio2022seeing}, while the other stresses the importance of low-level features within human visual biological mechanisms \citep{gori2016visual}.

Visual illusions can affect human behavior in multiple ways. Research has shown that human action cannot resist visual illusions \citep{gentilucci1996visual, franz2001action, carey2001action}, so is language comprehension and language production. Such findings catalyze inquiries regarding the capability of models to comprehend language instructions based on human perceptions and align them with human intent. The issue of human-AI alignment has gained considerable attention, emphasizing the development of agents behaving in consonance with user intentions \citep{leike2018scalable}. Investigating the visual illusion of language models provides an important perspective on the alignment between humans and machines regarding language communication.

\paragraph{Resources for Illusion Evaluation.}

Previous work made efforts to provide systematic data and tools to study visual illusion. Some work introduced tools to compute and generate illusory images systematically regarding the likelihood of patches and abutting grating distortion \cite{hirsch2020color, fan2023challenging}. \citet{makowski2021parametric} produced open-source software with a parametric framework to manipulate the generate illusions in a systematic way. Besides, \citet{gomez2022synthesis} proposed a framework synthesizing new visual illusions using the optimization abilities of current automatic differentiation techniques, which can be applied to vision models to understand the difference between vision models and human perception. These are earlier endeavors to establish a foundation for scalable and reproducible research on machine illusions. 

In accordance with these efforts, our study presents a unique contribution: we present the first dataset offering natural language annotations for the assessment of machine-processed visual illusions from a language-grounding viewpoint. The intent of this work is to bridge the current gap by fostering future evaluations of language models, specifically with respect to their alignment with human visual illusions.


\paragraph{Evaluation of Machine Visual Illusion.}
 Previous work \citep{gomez2019convolutional,gomez2020color,afifi2019else, benjamin2019shared} have shown convolutional neural networks trained on ImageNet or low-level vision tasks can be deceived by some kind of visual illusions as humans do in various degrees. Model scale and structure can affect the model’s response to visual illusion. \citet{gomez2020color} revealed that network illusions could be inconsistent with the perception of humans, and architectures with more complexity may have a worse capability in replicating human visual illusions. Some work focused on optimal information processing and revealed that optimized readouts of local visual orientation from the networks’ internal representations show similar illusions as human \citep{benjamin2019shared}.

While previous work focused solely on the vision model, our work takes language into consideration and contributes a new perspective. Visual illusion, as a psychological and biological activity of humans, is transferred and communicated through human language. Human language serves as an interface to interact with machines. Therefore, from the perspective of human language, our work helps better understand the alignment between machine and human perception and sheds light on future improvements in machine behavior.


\paragraph{Foundation Vision-Language Models.} 
Recent advancements in foundational vision-language models (VLMs) have shown impressive results across a broad spectrum of tasks~\cite{openai2023gpt4, wang2022ofa, lu2022unified, alayrac2022flamingo, clip}. These models, acting as user interfaces, interact with users through both language and visuals, necessitating a deep understanding of human intent and an alignment with human values to make them more useful.
While previous research has primarily focused on language-based uni-modal alignment problems~\cite{rlhf,kosinski2023tom}, our work offers a fresh perspective.  Centered on the intersection of VLM's perception capability and human cognitive biases, we investigate to what degree they can understand humans and align with human intentions under visual illusions.

==> _Table-results.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{Model}} & \multicolumn{4}{c|}{Task} \\ \cline{3-6} 
\multicolumn{2}{|c|}{} & Same-Diff QA & Subj QA & Desc QA & Localization \\ \hline
\multirow{4}{*}{OFA} & Tiny & 4.25 & 0.5 & 0.5 & 4.25 \\
 & Base & 19.5 & 7.5 & 3.0 & 11.25 \\
 & Large & 14.5 & 14.0 & 9.0 & 21.0 \\
 & Huge & 15.0 & 12.0 & 11.0 & 22.75 \\ \hline
\multirow{4}{*}{UIO} & Small & 8.25 & 2.75 & 2.25 & 9.0 \\
 & Base & 8.25 & 3.75 & 3.5 & 24.5 \\
 & Large & 28.75 & 7.75 & 11.25 & 27.75 \\
 & XL & 35.5 & 9.75 & 9.5 & 29.0 \\ \hline
\end{tabular}
\caption{Evaluation of different models on various tasks. Each score represents the "humanlike" attribute of the corresponding model on the specific task. Higher scores indicate more human-like responses.}
\label{tb:results}
\end{table*}


==> _Table-task-evaluations.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{.99\linewidth}{!}{
\begin{tabular}{m{0.04\linewidth} m{0.3\linewidth} m{0.32\linewidth} m{0.33\linewidth}}
\toprule
Task & Match & Mismatch & Self-Contradiction / Irrelevant \\
\midrule
SDQA 
& Consistently consider the objects as identical in the inducer-removed image and different in the illusion image
& Consistently consider the objects as identical in the inducer-removed image, while still identical in the illusion image
& Give the same response to both questions or consider the objects as different in the inducer-removed image \\
\midrule
SQA 
& Consistently select the object matching the illusionary description
& Consistently select the object opposite to the illusionary description
& Give the same response to both questions \\
\midrule
DQA 
& Consistently select the description matching with human illusion
& Consistently select the description opposite to human illusion
& Give the same response to both questions \\
\midrule
OL 
& Consistently localize the object described by the illusionary description
& Consistently localize the object in the opposite of the illusionary description
& Localize the same object / Cannot localize any object of interest \\
\bottomrule
\end{tabular}
}
\caption{Evaluation criteria for machine-human illusion alignment in the four tasks.  }
\label{tb:task_evals} 
\end{table*}
